The Mass-Loss Induced Eccentric Kozai Mechanism: A New Channel for the Production of Close Compact Object-Stellar Binaries

Over a broad range of initial inclinations and eccentricities an appreciable fraction of hierarchical triple star systems with similar masses are essentially unaffected by the Kozai-Lidov mechanism (KM) until the primary in the central binary evolves into a compact object. Once it does, it may be much less massive than the other components in the ternary, enabling the "eccentric Kozai mechanism (EKM):" the mutual inclination between the inner and outer binary can flip signs driving the inner binary to very high eccentricity, leading to a close binary or collision. We demonstrate this "Mass-loss Induced Eccentric Kozai" (MIEK) mechanism by considering an example system and defining an ad-hoc minimal separation between the inner two members at which tidal affects become important. For fixed initial masses and semi-major axes, but uniform distributions of eccentricity and cosine of the mutual inclination, ~10% of systems interact tidally or collide while the primary is on the MS due to the KM or EKM. Those affected by the EKM are not captured by earlier quadrupole-order secular calculations. We show that fully ~30% of systems interact tidally or collide for the first time as the primary swells to AU scales, mostly as a result of the KM. Finally, ~2% of systems interact tidally or collide for the first time after the primary sheds most of its mass and becomes a WD, mostly as a result of the MIEK mechanism. These findings motivate a more detailed study of mass-loss in triple systems and the formation of close NS/WD-MS and NS/WD-NS/WD binaries without an initial common envelope phase.

==> tab2.tex <==
\begin{deluxetable}{lllll}%[hpt]
\tablecolumns{5}
\tablewidth{0pc}
\tabletypesize{\scriptsize}
\tablecaption{Triple Outcomes}
\tablehead{
\colhead{} &
\colhead{Contact} &
\colhead{Flip} &
\colhead{Contact \& Flip} &
\colhead{Unbound} 
}
\startdata
{\bf  $ \rtide = 2.5 \ R_{*}$}  &              \\
$ \ \ \  \  $Primary MS & \TidalBeforeRtideless{} & \FlipBeforeRtideless{} & \TidalFlipBeforeRtideless{} &  \DistruptedBeforeRtideless{} \\
$ \ \ \  \  $Primary Giant & \TidalEvolveRtideless{} & \FlipEvolveRtideless{} & \TidalFlipEvolveRtideless{} & \DistruptedEvolveRtideless{} \\
$ \ \ \  \  $During Mass-Loss & \TidalDuringRtideless{} & \FlipDuringRtideless{} & \TidalFlipDuringRtideless{} & \DistruptedDuringRtideless{} \\
$ \ \ \ \   $After Mass-Loss & \TidalAfterRtideless{} & \FlipAfterRtideless{} & \TidalFlipAfterRtideless{} &  \DistruptedAfterRtideless{} \\
{\bf  $ \rtide = 3.5 \ R_{*}$}  &              \\
$ \ \ \  \  $Primary MS & \TidalBeforeRtidemore{} & \FlipBeforeRtidemore{} & \TidalFlipBeforeRtidemore{} &  \DistruptedBeforeRtidemore{} \\
$ \ \ \  \  $Primary Giant & \TidalEvolveRtidemore{} & \FlipEvolveRtidemore{} & \TidalFlipEvolveRtidemore{} & \DistruptedEvolveRtidemore{} \\
$ \ \ \  \  $During Mass-Loss & \TidalDuringRtidemore{} & \FlipDuringRtidemore{} & \TidalFlipDuringRtidemore{} & \DistruptedDuringRtidemore{} \\
$ \ \ \ \   $After Mass-Loss & \TidalAfterRtidemore{} & \FlipAfterRtidemore{} & \TidalFlipAfterRtidemore{} &  \DistruptedAfterRtidemore{} \\
{\bf  $ \rtide = 5 \ R_{*}$}  &              \\
$ \ \ \  \  $Primary MS & \TidalBeforeRtidefive{} & \FlipBeforeRtidefive{} & \TidalFlipBeforeRtidefive{} &  \DistruptedBeforeRtidefive{} \\
$ \ \ \  \  $Primary Giant & \TidalEvolveRtidefive{} & \FlipEvolveRtidefive{} & \TidalFlipEvolveRtidefive{} & \DistruptedEvolveRtidefive{} \\
$ \ \ \  \  $During Mass-Loss & \TidalDuringRtidefive{} & \FlipDuringRtidefive{} & \TidalFlipDuringRtidefive{} & \DistruptedDuringRtidefive{} \\
$ \ \ \ \   $After Mass-Loss & \TidalAfterRtidefive{} & \FlipAfterRtidefive{} & \TidalFlipAfterRtidefive{} &  \DistruptedAfterRtidefive{} \\
{\bf  $ \rtide = 10 \ R_{*}$}  &              \\
$ \ \ \  \  $Primary MS & \TidalBeforeRtideten{} & \FlipBeforeRtideten{} & \TidalFlipBeforeRtideten{} &  \DistruptedBeforeRtideten{} \\
$ \ \ \  \  $Primary Giant & \TidalEvolveRtideten{} & \FlipEvolveRtideten{} & \TidalFlipEvolveRtideten{} & \DistruptedEvolveRtideten{} \\
$ \ \ \  \  $During Mass-Loss & \TidalDuringRtideten{} & \FlipDuringRtideten{} & \TidalFlipDuringRtideten{} & \DistruptedDuringRtideten{} \\
$ \ \ \ \   $After Mass-Loss & \TidalAfterRtideten{} & \FlipAfterRtideten{} & \TidalFlipAfterRtideten{} &  \DistruptedAfterRtideten{} \\


\enddata
\tablecomments{Same as Table \ref{tab:ParmsOutcomes} except with various assumed tidal radii. 
Table discussed in \S\ref{sec:rtide}. 
}

\label{tab:ParmsOutcomesRtide}
\end{deluxetable}

